HumanGPS: Geodesic PreServing Feature for Dense Human Correspondences

In this paper, we address the problem of building dense correspondences between human images under arbitrary camera viewpoints and body poses. Prior art either assumes small motion between frames or relies on local descriptors, which cannot handle large motion or visually ambiguous body parts, e.g., left vs. right hand. In contrast, we propose a deep learning framework that maps each pixel to a feature space, where the feature distances reflect the geodesic distances among pixels as if they were projected onto the surface of a 3D human scan. To this end, we introduce novel loss functions to push features apart according to their geodesic distances on the surface. Without any semantic annotation, the proposed embeddings automatically learn to differentiate visually similar parts and align different subjects into an unified feature space. Extensive experiments show that the learned embeddings can produce accurate correspondences between images with remarkable generalization capabilities on both intra and inter subjects.

==> application.tex <==
\section{Applications}
\label{sec:apps}
In this section, we show our GPS feature can be integrated and improve many existing computer vision tasks.

\subsection{Optical Flow}
% We first integrate the human surface feature into optical flow methods.
% While our method does not assume or exploit the small motion assumption which has been widely adopted by optical flow methods, the GPS feature should still be beneficial in building correct flow for challenging cases, e.g. texture-less region, occasional large motion.

% With dense mapping from human pixels to surface of human body, we can also trivially compute correspondence of the same person between two frames via intermediate mapping. However, finding correspondence with nearest neighbor search can’t guarantee the smoothness of results. On the other hand, optical flow methods prefer to produce smooth estimation and directly regress correspondences.  We propose to incorporate human surface feature into current optical flow framework for robust and fine-grained correspondence estimation. 
An obvious application for GPS is to combine it with existing optical flow models for correspondence search between frames.
To show that, we integrate our feature to state-of-the-art optical flow methods PWC-Net \cite{sun2018pwc} and RAFT \cite{teed2020raft}.
Both methods consist of a siamese feature extractor and a follow up network to regress the flow.
We attach an additional feature extractor and pretrain it with our losses to provide GPS feature.
% We incorporate  into one of the state-of-the-art method PWC-Net.
% We add another feature extractor with the same structure as the original one in PWC-Net, and pretrain this branch with our novel loss functions.
The GPS feature is then combined with the output of the original feature extractor by element-wise mean and then fed into the remaining layers of the network.
% Then the whole network will be trained with optical flow loss.
% Those two branches of features are fused with element-wise mean operation for computing feature similarity.
% We keep the other part of the network the same as the original PWC-net for fair comparison, in which optical flow is predicted in a coarse-to-fine manner using feature pyramid, warping, and cost volume. 

The quantitative evaluation is shown in \Autoref{tab:optical_flow_aepe}.
For a fair comparison, we compare our model with their original network (pre-trained), one fine-tuned on our datasets and a version with increased capacity where we add additional feature extractors but without employing our loss functions (marked with $^*$).
Both models trained on generic optical flow does not perform well on our data, which possibly imply that our datasets contain much larger pose variations compared to typical optical flow tasks and thus more challenging.
Nevertheless, fine-tuning on our dataset reduces the error, and adding an additional feature extractor further improves the accuracy.
In contrast, using our loss function to supervise the additional feature extractor can significantly reduce the error metrics on all the intra and inter subject test sets.
This shows that while our GPS feature can be used directly via nearest neighbor search, we can significantly improve the performance if more computational budget is available to run optical flow networks.
It is worth mentioning that models with our feature generalizes better to the inter-subject test set compared to other methods.

% The evaluation is reported in Tab.\ref{tab:optical_flow_aepe}.
% PWC-Net trained for generic optical flow does not perform well on our data, which probably because our dataset contain much larger flow compared to typical optical flow.
% Nevertheless, finetuning PWC-Net effectively reduce the error, which shows the good capacity of PWC-Net.
% Adding an additional feature encoder (PWC-Net*) can further improve the performance but not much, indicating that simply increase model capacity is not effective.
% In contrast, using our loss function to supervise the additional feature extractor can significantly reduce the error metrics on all the intra and inter subject test set.
% This shows that our human surface feature can effectively improve optical flow quality.

Figure \ref{fig:vis_optical_flow} \todo{broken ref} shows qualitative results.
% \yd{show some qualitative results?}
% \yd{Add non-finetuned PWC-net to table.}
\yd{Evaluate on standard benchmark.}
\yd{Show number for different cases, e.g. occlusion, small/large motion.}

% commments:

% If we use PWC-Net, the performance on intra-subject data will decrease, but the performance on inter-subject data will increased where the model is train on intra-subject data. 

% We may move the evaluation of RAFT into supplementary and put the evaluation of PWC-Net here.

% Compared with SIFT feature by evaluating FlowFields++, CPM.

% Compared with SIFTFlow feature.

% Evaluate methods on a public dataset.

% When compared with RAFT*, do we need to use triplet loss.

% \begin{figure*}[t]
% \begin{center}
% \includegraphics[height=10cm, width=16cm]{example-image}
% \end{center}
% % \vspace{-0.4in}
% \caption{Visualize optical flow, and compared with other methods. There may be left-right ambiguities in other methods.
% }
% \label{fig:vis_optical_flow}
% \end{figure*}



\begin{table*}[t]
\centering

\begin{tabular}{|l|lll11111|}
\hline
% \multicolumn{1}{|c|}{Methods} & \multicolumn{4}{c|}{Accuracy} \\ 
% \cline{2-5}
\multicolumn{1}{|c|}{} & \multicolumn{6}{c|}{Intra} &   \multicolumn{2}{c|}{Inter} & 
\cline{2-9}
\multicolumn{1}{|c|}{Methods} & \multicolumn{2}{c|}{SMPL \cite{loper2015smpl}} & \multicolumn{2}{c|}{The Relightables \cite{guo2019relightables}}& \multicolumn{2}{c|}{RenderPeople \cite{renderpeople}} &   \multicolumn{2}{c|}{SMPL \cite{loper2015smpl}} &  
\cline{2-9}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{non} & \multicolumn{1}{c|}{all} & \multicolumn{1}{c|}{non}& \multicolumn{1}{c|}{all}&  \multicolumn{1}{c|}{non} &  \multicolumn{1}{c|}{all} &   \multicolumn{1}{c|}{non} &  \multicolumn{1}{c|}{all} &  \hline
PWC-Net pre-trained & 
\multicolumn{1}{l|}{{28.70}} & \multicolumn{1}{l|}{{39.51}} & \multicolumn{1}{c|}{{16.26}} & \multicolumn{1}{c|}{{21.44}} &  \multicolumn{1}{c|}{39.33} & \multicolumn{1}{c|}{46.51} & \multicolumn{1}{c|}{45.69}  & \multicolumn{1}{c|}{51.42}\\
\hline
PWC-Net fine-tuned & 
\multicolumn{1}{c|}{4.51} & \multicolumn{1}{c|}{13.27} & \multicolumn{1}{c|}{3.57} & \multicolumn{1}{c|}{10.01} & \multicolumn{1}{c|}{9.57} & \multicolumn{1}{c|}{18.74} &\multicolumn{1}{c|}{20.06} &\multicolumn{1}{c|}{28.14}
\\
\hline
PWC-Net* & 
\multicolumn{1}{c|}{3.89} & \multicolumn{1}{c|}{12.82} & \multicolumn{1}{c|}{3.42} &  \multicolumn{1}{c|}{9.39} & \multicolumn{1}{c|}{7.91}  & \multicolumn{1}{c|}{16.99}  & \multicolumn{1}{c|}{19.21}  & \multicolumn{1}{c|}{23.77}   \\ \hline
PWC-Net + GPS& 
\multicolumn{1}{c|}{2.73} & \multicolumn{1}{c|}{10.86} & \multicolumn{1}{c|}{2.99} &  \multicolumn{1}{c|}{9.01} & \multicolumn{1}{c|}{6.89}  & \multicolumn{1}{c|}{14.72}  & \multicolumn{1}{c|}{12.08}  & \multicolumn{1}{c|}{17.92}   \\ \hline
\hline
RAFT pre-trained  & 
\multicolumn{1}{c|}{27.14} & \multicolumn{1}{c|}{34.48} & \multicolumn{1}{c|}{15.23} & \multicolumn{1}{c|}{19.73} & \multicolumn{1}{c|}{40.16} & \multicolumn{1}{c|}{47.63} &\multicolumn{1}{c|}{51.76} &\multicolumn{1}{c|}{57.24}
\\
\hline
RAFT  fine-tuned & 
\multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{12.30} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{11.65} & \multicolumn{1}{c|}{6.74} & \multicolumn{1}{c|}{15.90} &\multicolumn{1}{c|}{45.47} &\multicolumn{1}{c|}{53.09}
\\
\hline
RAFT* & 
\multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{12.82} & \multicolumn{1}{c|}{2.79} &  \multicolumn{1}{c|}{11.39} & \multicolumn{1}{c|}{5.62}  & \multicolumn{1}{c|}{14.79}  & \multicolumn{1}{c|}{57.82}  & \multicolumn{1}{c|}{66.04}   \\ \hline
RAFT + GPS& 
\multicolumn{1}{c|}{2.13} & \multicolumn{1}{c|}{10.12} & \multicolumn{1}{c|}{2.27} &  \multicolumn{1}{c|}{10.52} & \multicolumn{1}{c|}{3.95}  & \multicolumn{1}{c|}{12.68}  & \multicolumn{1}{c|}{10.76}  & \multicolumn{1}{c|}{17.61}   \\ \hline
\hline

\end{tabular}
\caption{Quantitative evaluation on dense human correspondence via SOTA optical flow networks - PWC-Net \cite{sun2018pwc} and RAFT \cite{teed2020raft}. Models pre-trained for generic optical flow datasets do not perform well since our data contains large motion and challenging occlusion. On both architecture, integrating with our GPS feature achieve the best performance. See text for the $^*$ models. \yd{add a column for finetune and assign yes or no to each.}\yd{Bold the best.}}
\label{tab:optical_flow_aepe}
\vspace{-0.1in}
\end{table*}





% \begin{table*}[t]
% \centering
% \caption{Evaluate dense human correspondence by APEP metric on DenseHumanMatching dataset.}
% \begin{tabular}{|l|lll11111|}
% \hline
% % \multicolumn{1}{|c|}{Methods} & \multicolumn{4}{c|}{Accuracy} \\ 
% % \cline{2-5}
% \multicolumn{1}{|c|}{} & \multicolumn{6}{c|}{Intra} &   \multicolumn{2}{c|}{Inter} & 
% \cline{2-9}
% \multicolumn{1}{|c|}{Methods} & \multicolumn{2}{c|}{SMPL} & \multicolumn{2}{c|}{Holodeck}& \multicolumn{2}{c|}{RenderPeople} &   \multicolumn{2}{c|}{SMPL} &  
% \cline{2-9}
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{non} & \multicolumn{1}{c|}{all} & \multicolumn{1}{c|}{non}& \multicolumn{1}{c|}{all}&  \multicolumn{1}{c|}{non} &  \multicolumn{1}{c|}{all} &   \multicolumn{1}{c|}{non} &  \multicolumn{1}{c|}{all} &  \hline

% RAFT (without finetuning)  & 
% \multicolumn{1}{c|}{27.14} & \multicolumn{1}{c|}{34.48} & \multicolumn{1}{c|}{15.23} & \multicolumn{1}{c|}{19.73} & \multicolumn{1}{c|}{40.16} & \multicolumn{1}{c|}{47.63} &\multicolumn{1}{c|}{51.76} &\multicolumn{1}{c|}{57.24}
% \\
% \hline
% RAFT  & 
% \multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{12.30} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{11.65} & \multicolumn{1}{c|}{6.74} & \multicolumn{1}{c|}{15.90} &\multicolumn{1}{c|}{45.47} &\multicolumn{1}{c|}{53.09}
% \\
% \hline
% RAFT* & 
% \multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{12.82} & \multicolumn{1}{c|}{2.79} &  \multicolumn{1}{c|}{11.39} & \multicolumn{1}{c|}{5.62}  & \multicolumn{1}{c|}{14.79}  & \multicolumn{1}{c|}{57.82}  & \multicolumn{1}{c|}{66.04}   \\ \hline
% RAFT + Human Surface Feature& 
% \multicolumn{1}{c|}{2.13} & \multicolumn{1}{c|}{10.12} & \multicolumn{1}{c|}{2.27} &  \multicolumn{1}{c|}{10.52} & \multicolumn{1}{c|}{3.95}  & \multicolumn{1}{c|}{12.68}  & \multicolumn{1}{c|}{10.76}  & \multicolumn{1}{c|}{17.61}   \\ \hline

% \end{tabular}
% \label{tab:optical_flow_aepe}
% \vspace{-0.1in}
% \end{table*}


% \begin{table}[]
% \caption{Evaluate Optical Flow on DenseHumanMatching Dataset.(Train only on intra-subject data)}
% \begin{tabular}{|l|lll1|}
% \hline
% \multicolumn{1}{|c|}{Methods} & \multicolumn{4}{|c|}{Accuracy} \\ 
% \cline{2-5}
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{SMPL Intra} & \multicolumn{1}{c|}{Holodeck}& \multicolumn{1}{c|}{RP} &   \multicolumn{1}{c|}{SMPL Inter} &  \hline
% RAFT & \multicolumn{1}{l|}{{5.68}} & \multicolumn{1}{l|}{{4.63}} &  \multicolumn{1}{l|}{10.03} & \multicolumn{1}{l|}{46.18}\\
% \hline
% RAFT*  & \multicolumn{1}{l|}{5.51} & \multicolumn{1}{l|}{4.46} & \multicolumn{1}{l|}{9.83}       & \multicolumn{1}{l|}{50.02}
% \\
% \hline
% RAFT+SF & \multicolumn{1}{l|}{5.28} & \multicolumn{1}{l|}{4.21} & \multicolumn{1}{l|}{9.43}  & \multicolumn{1}{l|}{30.53}       \\ \hline
% \end{tabular}
% \label{tab:tang}
% \vspace{-0.1in}
% \end{table}


% \begin{table}[]
% \caption{Evaluate Optical Flow on DenseHumanMatching Dataset. (Trained both on intra- and inter- subject data)}
% \begin{tabular}{|l|lll1|}
% \hline
% \multicolumn{1}{|c|}{Methods} & \multicolumn{4}{|c|}{Accuracy} \\ 
% \cline{2-5}
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{SMPL Intra} & \multicolumn{1}{c|}{Holodeck}& \multicolumn{1}{c|}{RP} &   \multicolumn{1}{c|}{SMPL Inter} &  \hline
% RAFT & \multicolumn{1}{l|}{5.33} & \multicolumn{1}{l|}{4.84} &  \multicolumn{1}{l|}{9.34} & \multicolumn{1}{l|}{8.57}\\
% \hline
% RAFT*  & \multicolumn{1}{l|}{5.16} & \multicolumn{1}{l|}{4.20} & \multicolumn{1}{l|}{9.15}       & \multicolumn{1}{l|}{8.32}
% \\
% \hline
% RAFT+SF & \multicolumn{1}{l|}{5.02} & \multicolumn{1}{l|}{4.31} & \multicolumn{1}{l|}{8.03}  & \multicolumn{1}{l|}{9.12}       \\ \hline
% \end{tabular}
% \label{tab:tang}
% \vspace{-0.1in}
% \end{table}

\begin{table}[t]
\begin{tabular}{|l|lll|}
\hline
\multicolumn{1}{|c}{Methods} & \multicolumn{3}{|c|}{Accuracy}                                                                   \\ \cline{2-4}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{5 cm} & \multicolumn{1}{c|}{10 cm}&  \multicolumn{1}{c|}{20 cm}     \\ \hline
SMPLify~\cite{bogo2016keep} & \multicolumn{1}{l|}{20.73} & \multicolumn{1}{l|}{40.05} & 54.23  \\
\hline
DP ResNet-101 FCN \cite{guler2018densepose} & \multicolumn{1}{l|}{43.05} & \multicolumn{1}{l|}{65.23} & 74.17  \\
\hline
DP ResNet-101 FCN* \cite{guler2018densepose} & \multicolumn{1}{l|}{51.32} & \multicolumn{1}{l|}{75.50} & 85.76   \\
\hline
SlimDP HG - 1 stack  & \multicolumn{1}{l|}{49.89} & \multicolumn{1}{l|}{74.04} & 82.98\\
\hline
SlimDP HG - 2 stack  & \multicolumn{1}{l|}{52.23} & \multicolumn{1}{l|}{76.50} & 84.99\\
\hline
SlimDP HG - 8 stack  & \multicolumn{1}{l|}{56.04} & \multicolumn{1}{l|}{79.63} & 87.55\\
\hline
Our ResNet-101 FCN  & \multicolumn{1}{l|}{49.09} & \multicolumn{1}{l|}{73.12} & 84.51  \\ \hline
Our ResNet-101 FCN* & \multicolumn{1}{l|}{53.01} & \multicolumn{1}{l|}{76.77} & 87.70  \\ \hline
Our HG - 1- stack  & \multicolumn{1}{l|}{50.50} & \multicolumn{1}{l|}{75.57} & 87.18  \\ \hline
\end{tabular}
\caption{Quantitative evaluation for dense human pose regression on DensePose COCO dataset \cite{guler2018densepose}. Following previous work \cite{guler2018densepose}, we assume ground truth bounding box is given and calculate percentage of pixels with error smaller than thresholds. We also compare models train w/ and w/o background. \yd{Waiting for numbers.}}
\label{tab:geodesic_error}
\end{table}

\subsection{Dense Human Pose Regression}
An interesting byproduct of the GPS feature is that it automatically maps features extracted from different subjects to the same embedding, and thus applications such as dense human pose regression \cite{guler2018densepose}, directly benefit from this approach.
To fully show the effect of the GPS feature, we pretrain a GPS feature extractor on our dataset, attach two more MLP layers, and finetune on DensePose-COCO dataset \cite{guler2018densepose} to regress the UV coordinates.
To make sure the model capacity is comparable with other methods, we use the backbone of previous methods for feature extraction, i.e. an FCN in DensePose \cite{guler2018densepose}, and Hourglass in Slim DensePose \cite{neverova2019slim} \todo{missing numbers for these, check later}.
To compare strictly on the matching accuracy, we adopt the same evaluation setup as DensePose and Slim Densepose, where ground truth bounding box is given; percentages of pixels with geodesic error less than certain thresholds are taken as the metric; and evaluate on DensePose MSCOCO benchmark \cite{guler2018densepose}.
Table \ref{tab:geodesic_error} shows the comparison with previous work.
When considering the same network capacity, our method achieves consistently better performance than previous methods.
Note that the UV coordinates are estimated via only two layers of MLP, which indicates the GPS feature is effective at aligning different subjects.

Figure \todo{figure} shows a qualitative comparisons with DensePose by warping one image to the other using the correspondence built using UV space or our feature space \yd{still missing} \todo{comment this when fig appears}.
Note that DensePose does not preserve details on regions that are not continuous in their UV parameterization, in particular on the face.
In contrast, our method learns a smooth high dimensional feature space that produces in general reasonable dense correspondences across subjects, leading to more visually appealing warping results.

% the DensePose architecture -- a ResNet101, as the feature extractor, and  
% the MLP layer is finetuned on DensePose dataset with the feature extractor freezed.
% Therefore such a model could only perform well if the informative feature for cross-subject correspondence descriptor are learned already by the feature extractor.

% As to the papers related to face descriptor, we assess quantitatively how well our embeddings correspond to human surface UV. we experiment on MS-COCO DensePose dataset, a large-scale ground-truth dataset with image-to-surface correspondences manually annotated. Following the previous approach, we add two layer of MLP on top of our feature extractor as regressors to estimate UV coordinates and segmentation labels. In detail, we pretrained our feature extractor on DenseHumanMatching dataset with novel geodesic triplet loss, then  we freeze its parameters and only learn the regressors on MS-COCO DensePose dataset. 

% We evaluate the performance on the DensePose
% MSCOCO benchmark with standard benchmarks based on Geodesic Point Similarity (GPS) metrics, and the comparison to previous methods are shown in Tab. \ref{tab:densepose}.
% \yd{also show some qualitative results?}

\begin{table*}[]
\centering
\begin{tabular}{|l|lll1111111|}
\hline
\multicolumn{1}{|c|}{Methods} & \multicolumn{1}{c}{AP}  & \multicolumn{1}{c}{AP_{50}} & \multicolumn{1}{c}{AP_{75}}& \multicolumn{1}{c}{AP_M}& \multicolumn{1}{c}{AP_L}& \multicolumn{1}{c}{AR}& \multicolumn{1}{c}{AR_{50}}& \multicolumn{1}{c}{AR_{75}}& \multicolumn{1}{c}{AP_M}& \multicolumn{1}{c|}{AP_L} \\ 
\hline
DensePose (ResNet-101) & 
\multicolumn{1}{c|}{51.8}  & \multicolumn{1}{c|}{83.7} & \multicolumn{1}{c|}{56.3}& \multicolumn{1}{c|}{42.2}& \multicolumn{1}{c|}{53.8}& \multicolumn{1}{c|}{61.1}& \multicolumn{1}{c|}{ 88.9}& \multicolumn{1}{c|}{66.4}& \multicolumn{1}{c|}{45.3}& \multicolumn{1}{c|}{52.1}\\
% \hline
% Slim DP (ResNeXt101)  & \multicolumn{1}{c|}{55.5}  & \multicolumn{1}{c|}{89.1} & \multicolumn{1}{c|}{60.8}& \multicolumn{1}{c|}{50.7}& \multicolumn{1}{c|}{56.8}& \multicolumn{1}{c|}{63.2}& \multicolumn{1}{c|}{92.6}& \multicolumn{1}{c|}{69.6}& \multicolumn{1}{c|}{51.8}& \multicolumn{1}{c|}{64.0}\\
% \hline
% SimPose  & \multicolumn{1}{c|}{56.2}  & \multicolumn{1}{c|}{87.9} & \multicolumn{1}{c|}{65.3}& \multicolumn{1}{c|}{61.0}& \multicolumn{1}{c|}{58.0}& \multicolumn{1}{c|}{65.2}& \multicolumn{1}{c|}{95.1}& \multicolumn{1}{c|}{75.2}& \multicolumn{1}{c|}{63.2}& \multicolumn{1}{c|}{65.3}\\
\hline
Ours & 
\multicolumn{1}{c|}{54.9}  & \multicolumn{1}{c|}{90.3} & \multicolumn{1}{c|}{61.3}& \multicolumn{1}{c|}{50.8}& \multicolumn{1}{c|}{54.9}& \multicolumn{1}{c|}{64.2}& \multicolumn{1}{c|}{94.6}& \multicolumn{1}{c|}{70.8}& \multicolumn{1}{c|}{52.8}& \multicolumn{1}{c|}{61.3}     \\ 
\hline
\end{tabular}
\caption{Multi-person dense pose evaluation. We show standard metrics on DensePose benchmark. As bounding box detection is out of scope of this paper, we use the bounding box predicted from DensePose \cite{} and replace the UV regression model to ours. \yd{Numbers need to be verified.}}
\label{tab:densepose}
\vspace{-0.1in}
\end{table*}






\subsection{Occlusion Detection}
Occlusion detection is important for many applications such as stereo matching where often in real scenarios it is preferable to invalidate non-valid matches rather than hallucinate wrong disparity hypotheses.
As shown in previous section, the distance map of GPS feature can be used to indicate occluded pixels.
Here we further improve the occlusion detection performance by adding an additional layer in the output of the PWC-Net to regress an occlusion mask.
The regression part of the PWC-Net takes the cost-volume as input, which is a reasonable measurement of the feature distance.

The precision recall curve of occlusion detection is shown in Fig. \todo{xxx} \yd{still missing}, and the mean averaged error and average precision are shown in Tab. \ref{tab:pred_occlusion}.
Again, using our GPS feature achieves the best accuracy, compared to a pre-trained and a fined-tuned PWC-Net with increased capacity. Similarly, when we compare to other correspondence search methods such as SDC-Net \cite{schuster2019sdc} and Wei \etal \cite{wei2016dense}, our approach outperforms both the baselines.

% As evaluation metric, we calculate mean average error between the predicted occlusion likelihood and ground truth label, and the average precision of occlusion detection.
% Similar like optical flow, we compare to PWC-Net and PWC-Net*, and the quantitative evaluation is shown in Tab. \ref{tab:pred_occlusion}.
% Again, adding additional feature extractor improves the prediction accuracy, and training with our loss function further improve the performance.



\begin{table*}[t]
\centering
\begin{tabular}{|l|lll11111|}
\hline
% \multicolumn{1}{|c|}{Methods} & \multicolumn{4}{c|}{Accuracy} \\ 
% \cline{2-5}
\multicolumn{1}{|c|}{Methods} & \multicolumn{6}{c|}{Intra} &   \multicolumn{2}{c|}{Inter} & 
\cline{2-9}
\multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{SMPL} & \multicolumn{2}{c|}{Holodeck}& \multicolumn{2}{c|}{RenderPeople} &   \multicolumn{2}{c|}{SMPL} &  
\cline{2-9}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{AP} & \multicolumn{1}{c|}{MAE}& \multicolumn{1}{c|}{AP}&  \multicolumn{1}{c|}{MAE} &  \multicolumn{1}{c|}{AP} &   \multicolumn{1}{c|}{MAE} &  \multicolumn{1}{c|}{AP} &  \hline
SDC-Net \cite{schuster2019sdc}& 
\multicolumn{1}{c|}{null} & \multicolumn{1}{c|}{56.40} & \multicolumn{1}{c|}{null} &  \multicolumn{1}{c|}{48.17} & \multicolumn{1}{c|}{null}  & \multicolumn{1}{c|}{58.38}  & \multicolumn{1}{c|}{null}  & \multicolumn{1}{c|}{28.98}   \\ \hline

Wei \etal \cite{wei2016dense}& 
\multicolumn{1}{c|}{null} & \multicolumn{1}{c|}{32.20} & \multicolumn{1}{c|}{null} &  \multicolumn{1}{c|}{25.78} & \multicolumn{1}{c|}{null}  & \multicolumn{1}{c|}{34.13}  & \multicolumn{1}{c|}{null}  & \multicolumn{1}{c|}{32.25}   \\ \hline

Ours& 
\multicolumn{1}{c|}{null} & \multicolumn{1}{c|}{71.20} & \multicolumn{1}{c|}{null} &  \multicolumn{1}{c|}{56.08} & \multicolumn{1}{c|}{null}  & \multicolumn{1}{c|}{67.65}  & \multicolumn{1}{c|}{null}  & \multicolumn{1}{c|}{69.33}   \\ \hline
\hline
PWC-Net pre-trained & 
\multicolumn{1}{c|}{0.1181} & \multicolumn{1}{c|}{90.25} & \multicolumn{1}{c|}{0.1094} &  \multicolumn{1}{c|}{85.16} & \multicolumn{1}{c|}{0.1790}  & \multicolumn{1}{c|}{87.06}  & \multicolumn{1}{c|}{0.3243}  & \multicolumn{1}{c|}{72.18}   \\ \hline

PWC-Net*  & 
\multicolumn{1}{c|}{0.1023} & \multicolumn{1}{c|}{92.20} & \multicolumn{1}{c|}{0.1109} & \multicolumn{1}{c|}{85.33} & \multicolumn{1}{c|}{0.1631} & \multicolumn{1}{c|}{89.32} &\multicolumn{1}{c|}{0.3720} &\multicolumn{1}{c|}{63.06}\\
\hline

PWC-Net + GPS Feature& 
\multicolumn{1}{c|}{0.0875} & \multicolumn{1}{c|}{94.93} & \multicolumn{1}{c|}{0.1037} &  \multicolumn{1}{c|}{87.67} & \multicolumn{1}{c|}{0.1380}  & \multicolumn{1}{c|}{91.38}  & \multicolumn{1}{c|}{0.3210}  & \multicolumn{1}{c|}{80.91}   \\ \hline



\end{tabular}
\caption{Quantitative evaluation of occlusion detection. We show the mean average error and average precision for the occlusion detection on four test sets. If using feature distance directly as a measurement, our method significantly outperform other learning based descriptors. If combined with optical flow network, using our GPS feature can further improve over original architecture with similar capacity. \yd{bold the best, add up/down next to the metric showing which direction is better.}}
\label{tab:pred_occlusion}
\vspace{-0.1in}
\end{table*}


\subsection{Nonrigid Tracking and Fusion}
Existing nonrigid tracking/fusion systems~\cite{newcombe2015dynamicfusion,dou2016fusion4d,dou2017motion2fusion} have challenges when tracking fast motions.
Such a system typically employs the ICP alike method, and it requires a good initialization on the non-rigid deformation parameters to extract reliable point to point correspondences, which are in turn used to refine the deformation in an iterative manner. 
Human body movements such as waving arms would easily break above requirement when performed too fast. Whereas high speed cameras \cite{need4speed,twinfusion} could mitigate this behavior, here we show that GPS is also an effective way to improve the results without the need of custom hardware.

The correspondences from our learned human surface features on color images provides additional constraints for the nonrigid tracking system, and it helps to rescue ICP failures.
To demonstrate that, we provide correspondence built across $4$ color images as additional initialization for the nonrigid deformation along with the ICP.
As shown in Fig. \ref{fig:nonrigid_tracking_comparison}, the standard dynamic fusion system fails quickly under fast motion, whereas successfully track the deformation with our correspondences.

\begin{figure}
\center
\includegraphics[ width=8cm]{./figs/nonrigid-tracking-with-corrs.png}
\caption{Nonrigid Tracking Comparison. \emph{top}) tracking without learned correspondences; \emph{bottom}) tracking with learned correspondences.  \yd{Add color image?}
}
\label{fig:nonrigid_tracking_comparison}
\end{figure}

\subsection{4D Scan Alignment and Compression}
The correspondence can align the geometry and texture map (i.e. UV space) of 4D scans. This may potentially benefit the compression. \todo{finish this, show results or remove paragraph}.

\subsection{Morphing}

\todo{Describe results and refer to Fig \ref{fig:vis_inter}}
\begin{figure}
\center
\includegraphics[width=8cm]{./figs/inter_flow_result.jpg}
\caption{Morphing results on inter-subject data. We show the correspondence between different persons, and the warping of the 2nd image to the 1st image. Compared to DensePose using non-continuous UV space for correspondence, our warping results contain less artifacts due to the smooth feature space. \yd{missing densepose warping results}}
\label{fig:vis_inter}
\end{figure}

Morphing is a powerful technique to create smooth animation between images. The vital key to successful image morphing is to create a map that aligns corresponding image elements. \cite{liao2014automating,liao2014semi}. With GPS feature, one can directly establish pixels correspondences to create a smoother video transition. \todo{finish this, show images}

\todo{we promised AP for occlusions detection in the main paper}

\todo{We promised more in the wild results, perhaps comparisons with DensePose?}
